End-to-End Learning of Motion Representation for Video Understanding

Despite the recent success of end-to-end learned representations, hand-crafted optical flow features are still widely used in video analysis tasks. To fill this gap, we propose TVNet, a novel end-to-end trainable neural network, to learn optical-flow-like features from data. TVNet subsumes a specific optical flow solver, the TV-L1 method, and is initialized by unfolding its optimization iterations as neural layers. TVNet can therefore be used directly without any extra learning. Moreover, it can be naturally concatenated with other task-specific networks to formulate an end-to-end architecture, thus making our method more efficient than current multi-stage approaches by avoiding the need to pre-compute and store features on disk. Finally, the parameters of the TVNet can be further fine-tuned by end-to-end training. This enables TVNet to learn richer and task-specific patterns beyond exact optical flow. Extensive experiments on two action recognition benchmarks verify the effectiveness of the proposed approach. Our TVNet achieves better accuracies than all compared methods, while being competitive with the fastest counterpart in terms of features extraction time.

==> sec_tvl1_backup.tex <==
\section{Problem Setup}
Let $\Mat{I}$ denote an image of size $H\times W$. A video is defined as a image sequence $\mathbb{I}=\{\Mat{I}_i\}_{i=0}^T$. The coordinates of the pixels in image $\Mat{I}$ compose a grid denoted $\Omega$. For any point $\Vec{x}=(x,y)\in\Omega$,
let $\Mat{I}_t(\Vec{x})$ be the gray density at time $t$ and $(x(t), y(t))$ be the trajectory across the image sequence $\mathbb{I}$. The displacement vector between $(x(t), y(t))$ and $(x(t+1), y(t+1))$ defines the optical flow field $\Vec{u}(\Vec{x})=(\Vec{u}_1(\Vec{x}),\Vec{u}_2(\Vec{x}))$, where $\Vec{u}_1(\Vec{x})$ and $\Vec{u}_2(\Vec{x})$  correspond to the horizontal and vertical directions, respectively.


\begin{figure*}[!th]
\begin{center}
\subfigure{
\includegraphics[width=2\columnwidth]{tvnet_new}
}
\caption{(a) The multi-scale version of the TV-L1 method. Here the scale-size, \ie $N_{scales}$ is 3. (b) The illustration of the process for unfolding TV-L1 to TVNet. Here, we only illustrate the while-loop of Algorithm~\ref{Alg:tvl1} for simplicity. Given two consecutive images $\Vec{I}_0$ and $\Vec{I}_1$, we iteratively compute the immediate variables $\Mat{I}_1(\Vec{x}+\Vec{u}^0), \nabla\Mat{I}_1(\Vec{x}+\Vec{u}^0), \Vec{v}, \Vec{p}$ and the optical flow $\Vec{u}$. The computations related to $\Vec{v}, \Vec{p}$ and $\Vec{u}$ is called recursively. The updates denoted as red line is parameterized by certain parameters which can be fine-tuned by end-to-end training. (c) The end-to-end model for action recognition. }
%\setlength{\belowcaptionskip}{0cm}
\label{Fig:tvnet}
\end{center}
\end{figure*}

\section{TVL1 method}
\label{Sec:tvl1}
To compute the optical flow $\Mat{u}(\Vec{x})$ between two consecutive images $\Mat{I}_0$ and $\Mat{I}_1$, the TV-L1 method~\cite{zach2007duality} is based on the brightness and smoothness constancy assumptions~\cite{horn1981determining}. In particular, it minimizes the total variations over all pixels $\Vec{x}$,
\begin{eqnarray}
\label{Eq:energy-function}
\min_{\Mat{u}(\Vec{x})} \sum_{\Vec{x}\in \Omega} (|\nabla \Vec{u}_1(\Vec{x})|+|\nabla \Vec{u}_2(\Vec{x})|) + \lambda|\rho(\Vec{u}(\Vec{x}))|,
\end{eqnarray}
where the first term $|\nabla \Vec{u}_1|+|\nabla \Vec{u}_2|$ accounts for the \emph{smoothness condition}, while the second term $|\rho(\Vec{u})|$ is for the \emph{brightness constancy assumption} \footnote{For convenience, we will omit the coordinate $\Vec{x}$ for $\Vec{u}(\Vec{x})$ henceforth if no ambiguity arises.}.
%The idea to optimize both the smoothness and brightness terms is dated back to . The difference made by TV-L1 is that it replaces the quadratic penalties with $\ell_1$ norms.
The second term given by $\rho(\Vec{u})=\Mat{I}_1(\Vec{x}+\Vec{u})-\Mat{I}_0(\Vec{x})$ is to penalize the brightness difference. Since $\Mat{I}_1(\Vec{x}+\Vec{u})$ is non-linear with respect to $\Vec{u}$, the authors in~\cite{zach2007duality} approximate $\rho(\Vec{u})$ by applying a Taylor expansion at an initial input $\Vec{u}^{0}$, hence leading to, $\rho(\Vec{u})=\nabla\Mat{I}_1(\Vec{x}+\Vec{u}^{0})(\Vec{u}-\Vec{u}^{0}) + \Mat{I}_1(\Vec{x}+\Vec{u}^0) -\Mat{I}_0(\Vec{x})$.

The authors further involve an auxiliary variable $\Vec{v}$ in Eq.~\eqref{Eq:energy-function} to enable a convex relaxation, \ie, \begin{eqnarray}
\label{Eq:convex-relaxation}
\min_{\Mat{u},\Mat{v}} \sum_{\Vec{x}\in \Omega} (|\nabla \Vec{u}_1|+|\nabla \Vec{u}_2|) + \frac{1}{2\theta}|\Vec{u}-\Vec{v}|^2 + \lambda|\rho(\Vec{v})|,
\end{eqnarray}
where a very small $\theta$ can force $\Vec{u}$ and $\Vec{v}$ to be equal at the minimum. This objective is minimized by alternatively updating $\Vec{u}$ and $\Vec{v}$. The details for the optimization process are presented in Algorithm~\ref{Alg:tvl1}, where the variables $\Vec{p}_1$ and $\Vec{p}_2$ are the dual flow vector fields.

\begin{algorithm}[h]
\caption{The TV-L1 method for optical flow extraction.}
\label{Alg:tvl1}
\begin{algorithmic}
   \STATE {\bfseries Hyper-parameters:} $\lambda,\theta,\tau,\epsilon,N_{warps},N_{iters}$
   \STATE {\bfseries Input:} $\Mat{I}_0,\Mat{I}_1,\Vec{u}^0$
   \STATE $\Vec{p}_1=[\Vec{p}_{11},\Vec{p}_{12}]=[\Vec{0},\Vec{0}]$;
   \STATE $\Vec{p}_2=[\Vec{p}_{21},\Vec{p}_{22}]=[\Vec{0},\Vec{0}]$;
   \FOR{$w=1$ {\bfseries to} $N_{warps}$}
   \STATE Warp $\Mat{I}_1(\Vec{x}+\Vec{u}^0), \nabla\Mat{I}_1(\Vec{x}+\Vec{u}^0)$ by interpolation;
   \STATE $\rho(\Vec{u})=\nabla\Mat{I}_1(\Vec{x}+\Vec{u}^{0})(\Vec{u}-\Vec{u}^{0})+\Mat{I}_1(\Vec{x}+\Vec{u}^0)-\Mat{I}_0(\Vec{x})$;
   \STATE $n=0$;
   \WHILE{$n<N_{iters}$ and ${stopping\_criterion}>\epsilon$}
   \STATE $\Vec{v}= \left\{
   \begin{array}{ll}
   \lambda\theta\nabla\Mat{I}_1 & \rho(\Vec{u})<-\lambda\theta|\nabla\Mat{I}_1|^2,\\
   -\lambda\theta\nabla\Mat{I}_1 & \rho(\Vec{u})>\lambda\theta|\nabla\Mat{I}_1|^2,\\
   -\rho(\Vec{u})\frac{\nabla\Mat{I}_1}{|\nabla\Mat{I}_1|^2} & \text{otherwise},
   \end{array}
   \right. $ where $\nabla\Mat{I}_1$ represents $\nabla\Mat{I}_1(\Vec{x}+\Vec{u}^0)$ for short;
   \STATE $\Vec{u}_d=\Vec{v}+\theta \mathrm{div}(\Vec{p}_d)$, $d=1,2$;
   \STATE $\Vec{p}_d=\frac{\Vec{p}_d+\tau/\theta \nabla\Vec{u}_d}{1+\tau/\theta|\nabla\Vec{u}_d|}$, $d=1,2$;
   \STATE $n=n+1$;
   \ENDWHILE
   \ENDFOR
\vskip -0.1in
\end{algorithmic}
\end{algorithm}

In addition to the arithmetic operations (\eg, the matrix addition and multiplication), the core implementation of Algorithm~\ref{Alg:tvl1} involves the non-trivial computations for the \emph{gradients} (\ie, $\nabla\Mat{I}_1$ and $\nabla\Vec{u}_d$), \emph{divergence} (\ie, $div(\Vec{p})$), and \emph{warping} (\ie, $\Mat{I}_1$ and $\nabla\Mat{I}_1$).
%In particular, The central and forward differences are adopted to compute the gradients $\nabla\Mat{I}_1(\Vec{x}+\Vec{u}^0)$ and $\nabla\Vec{u}_d$, respectively; the backward difference is applied to compute the divergence $\mathrm{div}(\Vec{p}_d)$; the bicubic interpolation [] is applied to warp the image $\Mat{I}_1$ by a flow field $\Vec{u}^0$.
The details of the numerical computations are provided as follows.
%Note that the Neumann boundary condition is used for the boundary points.
\begin{itemize}
  \item The gradient of the image $\Mat{I}_1$ is computed by central difference:
  \begin{eqnarray}
  \label{Eq:central}
  \frac{\partial \Mat{I}_1(i,j)}{\partial x} = \left\{
   \begin{array}{ll}
   \frac{\Mat{I}_1(i+1,j)-\Mat{I}_1(i-1,j)}{2} & 1<i<W,\\
   0 & \text{otherwise}.
   \end{array}
   \right.
  \end{eqnarray}
  We can similarly compute $\frac{\partial}{\partial y} \Mat{I}_1(i,j)$ along the $j$ index.
  \item The gradient of each component of the flow $\Mat{u}$ is computed via the forward difference:
  \begin{eqnarray}
  \label{Eq:forward}
  \frac{\partial \Vec{u}_d(i,j)}{\partial x} = \left\{
   \begin{array}{ll}
   \Vec{u}_d(i+1,j)-\Vec{u}_d(i,j) & 1\leq i<W,\\
   0 & \text{otherwise},
   \end{array}
   \right.
  \end{eqnarray}
  where $d\in\{1,2\}$. Also, $\frac{\partial}{\partial y} \Mat{u}_d(i,j)$ can be similarly computed by taking the difference on the $j$ index.
  \item The divergence of the dual variables $\Vec{p}$ is computed via the backward difference:
  \begin{eqnarray}
  \label{Eq:backward}
   \nonumber
   && \mathrm{div}(\Vec{p}_d)(i,j) \\
   \nonumber
   &=& \left\{
   \begin{array}{ll}
   \Vec{p}_{d1}(i,j)-\Vec{p}_{d1}(i-1,j) & 1< i <W,\\
   \Vec{p}_{d1}(i,j)  & i=1,\\
   -\Vec{p}_{d1}(i-1,j)  & i=W.
   \end{array}
   \right.\\
   &+&
   \left\{
   \begin{array}{ll}
   \Vec{p}_{d2}(i,j)-\Vec{p}_{d2}(i,j-1) & 1< j <H,\\
   \Vec{p}_{d2}(i,j)  & j=1,\\
   -\Vec{p}_{d2}(i,j-1)  & j=H.
   \end{array}
   \right.
  \end{eqnarray}
  \item Bicubic interpolation~\cite{horn1981determining} is used to warp the image $\Mat{I}_1$ by a flow field $\Vec{u}^0$, \ie, computing $\Mat{I}_1(\Vec{x}+\Vec{u}^0)$.
\end{itemize}

Since the Taylor expansion is applied to linearize the brightness difference, the initial flow field $\Vec{u}^0$ should be close the real field $\Vec{u}$ to ensure a small approximation error. To achieve this, the approximation field $\Vec{u}^0$ is effectively derived by a multi-scale scheme in a coarse-to-fine way. To be specific, at the coarsest level, $\Vec{u}^0$ is initialized as the zero vector and the optimized output is applied as the initialization of the next level.
Figure~\ref{Fig:tvnet} demonstrates the framework of TV-L1 with the number of scales being $N_{scales}=3$.



